Efficient inference of interventional distributions

We consider the problem of efficiently inferring interventional distributions in a causal Bayesian network from a finite number of observations. Let $\mathcal{P}$ be a causal model on a set $\mathbf{V}$ of observable variables on a given causal graph $G$. For sets $\mathbf{X},\mathbf{Y}\subseteq \mathbf{V}$, and setting ${\bf x}$ to $\mathbf{X}$, let $P_{\bf x}(\mathbf{Y})$ denote the interventional distribution on $\mathbf{Y}$ with respect to an intervention ${\bf x}$ to variables ${\bf x}$. Shpitser and Pearl (AAAI 2006), building on the work of Tian and Pearl (AAAI 2001), gave an exact characterization of the class of causal graphs for which the interventional distribution $P_{\bf x}({\mathbf{Y}})$ can be uniquely determined. We give the first efficient version of the Shpitser-Pearl algorithm. In particular, under natural assumptions, we give a polynomial-time algorithm that on input a causal graph $G$ on observable variables $\mathbf{V}$, a setting ${\bf x}$ of a set $\mathbf{X} \subseteq \mathbf{V}$ of bounded size, outputs succinct descriptions of both an evaluator and a generator for a distribution $\hat{P}$ that is $\varepsilon$-close (in total variation distance) to $P_{\bf x}({\mathbf{Y}})$ where $Y=\mathbf{V}\setminus \mathbf{X}$, if $P_{\bf x}(\mathbf{Y})$ is identifiable. We also show that when $\mathbf{Y}$ is an arbitrary set, there is no efficient algorithm that outputs an evaluator of a distribution that is $\varepsilon$-close to $P_{\bf x}({\mathbf{Y}})$ unless all problems that have statistical zero-knowledge proofs, including the Graph Isomorphism problem, have efficient randomized algorithms.

==> checklist.tex <==
\section*{Checklist}


\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    {\answerYes{See Sections~\ref{sec:eval},~\ref{sec:samp} and~\ref{sec:hard}}}
  \item Did you describe the limitations of your work?
    \answerYes{See discussions after Theorem 1.1.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See our theorem statements in the Introduction.}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{See Section~\ref{sec:eval},~\ref{sec:samp},~\ref{sec:hard} and Appendices.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNA{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> older.tex <==
Now we focus on learning $R=\prod_{i,j} R_{ij}$, where $R_{ij}:=P(\ve{C_{ij}} \mid \cdo(\ve{c_i}\setminus\ve{c_{ij}}))$. Each $R_{ij}$ takes a recursive call from Step 4 ??? with the original graph $G$ and the original distribution $P$. Recursive calls happen from steps 2, 4, and 7. Let $Q$ and $D$ be the distributions before and after taking a particular recursive call.  We refer to a recursive call {\em original}, if $Q=P$ (i.e. the distribution before is the original joint distribution) and {\em unoriginal} otherwise. With finite samples, we would be working with sufficiently close multiplicative approximations for $Q$ and $D$. The following inductive procedure gives an approximate distribution $\wh{D}$ for $D$, assuming an access to $\wh{Q}$ for $Q$.

\textcolor{red}{To be pseudocoded.}
\begin{enumerate}
    \item Step 2 and 4: $\widehat{D} \gets \widehat{Q}$ (in particular, original remains original).
    \item Step 7, `original case': learn each conditional factor of $D$ of step 7, up to $(1\pm\eps)$-factor using enough samples from $P$.
    \item Step 7, `unoriginal case': learn each conditional factor $D(A \mid \ve{B})=D(A\ve{B})/D(\ve{B})$ up to $(1\pm 3\eps)$-factor by appropriate marginalizations of $Q$ and taking ratios (no samples needed). 
\end{enumerate}
  
Clearly, $\widehat{D}=D$ for the original calls by induction. We show the following approximation guarantees for $\wh{D}$ about the unoriginal calls. 
\begin{claim}\label{claim:recLoss}
For an unoriginal call, if $\wh{Q}$ is a $(1\pm\eps)$-approx. of $Q$, then $\wh{D}$ is a $\approx(1\pm k\eps)$-approx. for $D$.
\end{claim}
\begin{proof}
In Steps 2 and 4, approximation ratio of $(1\pm\eps)$ is retained.

In either of the two cases for step 7, each conditional factor is $(1\pm3\eps)$-approx. Since there are at most $k$ conditional factors, the final approx. ratio is $\approx(1\pm \eps k)$
\end{proof}

Next, we analyze the terminal recursive calls, which generates the required formula from steps 1 or 6. We combine the appropriate terms to get $\wh{R}_{ij}$, an approx. for $R_{i,j}$.
\begin{claim}
For a terminal recursive call, the generated formula for this call is $(1\pm\eps k^{k+1})$-approx. of the true formula. 
\end{claim}
\begin{proof}
Step 1 is a marginalization, and hence do not lose approximation. For step 6. if we start with a $(1\pm\eps)$-approx., the final approximation would be $\approx(1\pm\eps k)$ using an argument similar to that of Claim~\ref{claim:recLoss}.

At recursion depth $j$, $\wh{Q}$ is $(1\pm\eps k^j)$-approx. of $Q$. Therefore, the ratio of each term of the final formula is $(1\pm\eps k^k)$, since the depth of recursion is at most $k$. The result follows since there are at most $k$ multiplications in the final formula. Step 2 is a marginalization and hence does not lose approx. factors. 
\end{proof}
